Bounding Duality Gap for Separable Problems with Linear Constraints

We consider the problem of minimizing a sum of non-convex functions over a compact domain, subject to linear inequality and equality constraints. Approximate solutions can be found by solving a convexified version of the problem, in which each function in the objective is replaced by its convex envelope. We propose a randomized algorithm to solve the convexified problem which finds an $\epsilon$-suboptimal solution to the original problem. With probability one, $\epsilon$ is bounded by a term proportional to the maximal number of active constraints in the problem. The bound does not depend on the number of variables in the problem or the number of terms in the objective. In contrast to previous related work, our proof is constructive, self-contained, and gives a bound that is tight.

==> invest2.tex <==
10 10 0.43
10 20 0.6150252525252525
10 30 0.7582654600301656
10 40 0.7827352472089312
10 50 0.8027045460932924
10 60 0.8445378344228779
10 70 0.8543746286393346
10 80 0.8838192925118606
10 90 0.9107681143233245
10 100 0.9012921179444613

20 10 1.0
20 20 0.3552777777777765
20 30 0.5182646520146499
20 40 0.6282911825017088
20 50 0.6986153846153846
20 60 0.7337609970674479
20 70 0.739353676985256
20 80 0.783953525204234
20 90 0.827086698509191
20 100 0.843120355131278

30 10 1.0
30 20 1.0
30 30 0.34505494505494505
30 40 0.44000000000000006
30 50 0.558
30 60 0.5949798387096773
30 70 0.667863916548127
30 80 0.7122369878183833
30 90 0.7437198581560284
30 100 0.7556092370243312

40 10 1.0
40 20 1.0
40 30 0.0
40 40 0.31605263157894736
40 50 0.4033333333333333
40 60 0.5092473118279569
40 70 0.5617460317460317
40 80 0.6066782810685251
40 90 0.6617156182547026
40 100 0.687496640326829

50 10 1.0
50 20 1.0
50 30 0.0
50 40 0.0
50 50 0.3401666666666666
50 60 0.40586206896551724
50 70 0.5053968253968253
50 80 0.5538414634146341
50 90 0.5948658649398704
50 100 0.6125188536953242

60 10 1.0
60 20 1.0
60 30 0.0
60 40 0.0
60 50 0.0
60 60 0.3260919540229884
60 70 0.3994957983193277
60 80 0.4725
60 90 0.4976811594202898
60 100 0.5393288084464553

70 10 1.0
70 20 0.0
70 30 0.0
70 40 0.0
70 50 0.0
70 60 0.0
70 70 0.3326890756302521
70 80 0.3975
70 90 0.45884057971014497
70 100 0.4754117647058823

80 10 1.0
80 20 0.0
80 30 0.0
80 40 0.0
80 50 0.0
80 60 0.0
80 70 0.0
80 80 0.34198717948717905
80 90 0.3524747474747475
80 100 0.43999999999999995

90 10 1.0
90 20 0.0
90 30 0.0
90 40 0.0
90 50 0.0
90 60 0.0
90 70 0.0
90 80 0.0
90 90 0.3279797979797979
90 100 0.3613877551020407

100 10 1.0
100 20 0.0
100 30 0.0
100 40 0.0
100 50 0.0
100 60 0.0
100 70 0.0
100 80 0.0
100 90 0.0
100 100 0.3183673469387755
